Hybrid Diffusion: Spectral-Temporal Graph Filtering for Manifold Ranking

State of the art image retrieval performance is achieved with CNN features and manifold ranking using a k-NN similarity graph that is pre-computed off-line. The two most successful existing approaches are temporal filtering, where manifold ranking amounts to solving a sparse linear system online, and spectral filtering, where eigen-decomposition of the adjacency matrix is performed off-line and then manifold ranking amounts to dot-product search online. The former suffers from expensive queries and the latter from significant space overhead. Here we introduce a novel, theoretically well-founded hybrid filtering approach allowing full control of the space-time trade-off between these two extremes. Experimentally, we verify that our hybrid method delivers results on par with the state of the art, with lower memory demands compared to spectral filtering approaches and faster compared to temporal filtering.

==> deriv-inv-v1.tex <==
\subsection{Derivation \alert{(version 1: inverse only)}}

We begin with the eigenvalue decomposition $\cW = U \Lambda U^\T$, which we partition as $\Lambda = \diag(\Lambda_1, \Lambda_2)$ and $U = (U_1 \ U_2)$. Matrices $\Lambda_1$ and $\Lambda_2$ are diagonal $r \times r$ and $(n-r) \times (n-r)$, respectively. Matrices $U_1$ and $U_2$ are $n \times r$ and $n \times (n-r)$, respectively, and have the following orthogonality properties, all due to the orthogonality of $U$ itself:
%
\begin{equation}
	U_1^\T U_1 = I_r, \quad U_2^\T U_2 = I_{n-r}, \quad
	U_1^\T U_2 = \vO, \quad U_1 U_1^\T + U_2 U_2^\T = I_n.
\label{eq:ortho}
\end{equation}
%
Then, $\cW$ is decomposed as
%
\begin{equation}
	\cW = U_1 \Lambda_1 U_1^\T + U_2 \Lambda_2 U_2^\T.
\label{eq:w-decomp}
\end{equation}
%
Similarly, $h_\alpha(\cW)$ is decomposed as
%
\begin{align}
	h_\alpha(\cW)
		& = U h_\alpha(\Lambda) U^\T
			\label{eq:h-decomp-1} \\
		& = U_1 h_\alpha(\Lambda_1) U_1^\T + U_2 h_\alpha(\Lambda_2) U_2^\T,
			\label{eq:h-decomp-2}
\end{align}
%
which is due to the fact that diagonal matrix $h_\alpha(\Lambda)$ is obtained by element-wise application, hence decomposed as $h_\alpha(\Lambda) = \diag(h_\alpha(\Lambda_1), h_\alpha(\Lambda_2))$. Here the first term is exactly the low-rank approximation that is used by spectral filtering, and the second is the approximation error
%
\begin{align}
	e_\alpha(\cW)
		& \defn U_2 h_\alpha(\Lambda_2) U_2^\T
			\label{eq:error-1} \\
		& = (1 - \alpha) U_2 (I_{n-r} - \alpha \Lambda_2)^{-1} U_2^\T
			\label{eq:error-2} \\
		& = (1 - \alpha) \left(
				\left( I_n - \alpha U_2 \Lambda_2 U_2^\T \right)^{-1} - U_1 U_1^\T
			\right)
			\label{eq:error-3} \\
		& = h_\alpha(U_2 \Lambda_2 U_2^\T) - (1 - \alpha) U_1 U_1^\T.
			\label{eq:error-4}
\end{align}
%
We have used the definition~(\ref{eq:transfer}) of $h_\alpha$ in~(\ref{eq:error-2}) and~(\ref{eq:error-4}). Equation~(\ref{eq:error-3}) can be verified by direct multiplication
%
\begin{align}
	& \left( U_1 U_1^\T + U_2 (I_{n-r} - \alpha \Lambda_2)^{-1} U_2^\T \right)
		(I_n - \alpha U_2 \Lambda_2 U_2^\T)
			\label{eq:verify-1} \\
	& = U_1 U_1^\T +
	    U_2 (I_{n-r} - \alpha\Lambda_2)^{-1} U_2^\T -
	    U_2 (I_{n-r} - \alpha\Lambda_2)^{-1} \alpha\Lambda_2 U_2^\T
			\label{eq:verify-2} \\
	& = U_1 U_1^\T +
	    U_2 (I_{n-r} - \alpha\Lambda_2)^{-1} (I_{n-r} - \alpha\Lambda_2) U_2^\T
			\label{eq:verify-3} \\
	& = U_1 U_1^\T + U_2 U_2^\T
			\label{eq:verify-4} \\
	& = I_n,
		\label{eq:verify-6}
\end{align}
%
where we have used the orthogonality properties~(\ref{eq:ortho}) in the expansion~(\ref{eq:verify-2}) and in~(\ref{eq:verify-6}). A similar verification holds for the opposite order of multiplication.

Now, combining~(\ref{eq:h-decomp-2}),~(\ref{eq:error-4}) and~(\ref{eq:w-decomp}), we have proved the following.

\begin{theorem}
	Assuming the definition~(\ref{eq:transfer}) of transfer function $h_\alpha$ and the eigenvalue decomposition~(\ref{eq:w-decomp}) of the symmetrically normalized adjacency matrix $\cW$, $h_\alpha(\cW)$ is decomposed as
	%
	\begin{equation}
		h_\alpha(\cW) = U_1 g_\alpha(\Lambda_1) U_1^\T + h_\alpha(\cW - U_1 \Lambda_1 U_1^\T),
	\label{eq:main}
	\end{equation}
	%
	where
	%
	\begin{equation}
		g_\alpha(A) \defn (1 - \alpha) \left( (I_n - \alpha A)^{-1} - I_n \right)
	\label{eq:aux}
	\end{equation}
	%
	for $n \times n$ real symmetric matrix $A$. For $x \in \real$ in particular, $g_\alpha(x) \defn  (1 - \alpha) \alpha x / (1 - \alpha x)$.
\end{theorem}



==> deriv-series-v1.tex <==
\subsection{Derivation \alert{(version 2: series)}}

We begin with the eigenvalue decomposition $\cW = U \Lambda U^\T$, which we partition as $\Lambda = \diag(\Lambda_1, \Lambda_2)$ and $U = (U_1 \ U_2)$. Matrices $\Lambda_1$ and $\Lambda_2$ are diagonal $r \times r$ and $(n-r) \times (n-r)$, respectively. Matrices $U_1$ and $U_2$ are $n \times r$ and $n \times (n-r)$, respectively, and have the following orthogonality properties, all due to the orthogonality of $U$ itself:
%
\begin{equation}
	U_1^\T U_1 = I_r, \quad U_2^\T U_2 = I_{n-r}, \quad
	U_1^\T U_2 = \vO, \quad U_1 U_1^\T + U_2 U_2^\T = I_n.
\label{eq:2-ortho}
\end{equation}
%
Then, $\cW$ is decomposed as
%
\begin{equation}
	\cW = U_1 \Lambda_1 U_1^\T + U_2 \Lambda_2 U_2^\T.
\label{eq:2-w-decomp}
\end{equation}
%
Now, as in~\cite{IAT+18}, we generalize $h_\alpha$ to any function $h$ that has a series expansion
%
\begin{equation}
	h(A) = \sum_{i=0}^\infty c_i A^i.
\label{eq:series}
\end{equation}
%
Then, assuming that $h(\cW)$ converges absolutely, it is similarly decomposed as
%
\begin{align}
	h(\cW)
		& = U h(\Lambda) U^\T
			\label{eq:2-h-decomp-1} \\
		& = U_1 h(\Lambda_1) U_1^\T + U_2 h(\Lambda_2) U_2^\T,
			\label{eq:2-h-decomp-2}
\end{align}
%
which is due to the fact that diagonal matrix $h_\alpha(\Lambda)$ is obtained by element-wise application, hence decomposed as $h_\alpha(\Lambda) = \diag(h_\alpha(\Lambda_1), h_\alpha(\Lambda_2))$. Here the first term is exactly the low-rank approximation that is used by spectral filtering, and the second is the approximation error
%
\begin{align}
	e_\alpha(\cW)
		& \defn U_2 h(\Lambda_2) U_2^\T
			\label{eq:2-error-1} \\
		& = \sum_{i=0}^\infty c_i U_2 \Lambda_2^i U_2^\T
			\label{eq:2-error-2} \\
		& = \sum_{i=0}^\infty c_i \left( U_2 \Lambda_2 U_2^\T \right)^i - c_0 U_1 U_1^\T
			\label{eq:2-error-3} \\
		& = h(U_2 \Lambda_2 U_2^\T) - h(0) U_1 U_1^\T.
			\label{eq:2-error-4}
\end{align}
%
We have used the series expansion~(\ref{eq:series}) of $h$ in~(\ref{eq:2-error-2}) and~(\ref{eq:2-error-4}). Equation~(\ref{eq:2-error-3}) is due to the fact that
%
\begin{equation}
	(U_2 \Lambda_2 U_2^\T)^i = U_2 \Lambda_2^i U_2^\T
\label{eq:term-pos}
\end{equation}
%
for $i \ge 1$, as can be verified by induction, while for $i = 0$,
%
\begin{equation}
	U_2 \Lambda_2^0 U_2^\T = U_2 U_2^\T = I_n - U_1 U_1^\T = (U_2 \Lambda_2 U_2^\T)^0 - U_1 U_1^\T.
\label{eq:term-zero}
\end{equation}
%
In both~(\ref{eq:term-pos}) and~(\ref{eq:term-zero}) we have used the orthogonality properties~(\ref{eq:2-ortho}).

Now, combining~(\ref{eq:2-h-decomp-2}),~(\ref{eq:2-error-4}) and~(\ref{eq:2-w-decomp}), we have proved the following.

\begin{theorem}
	Assuming the series expansion~(\ref{eq:series}) of transfer function $h$ and the eigenvalue decomposition~(\ref{eq:2-w-decomp}) of the symmetrically normalized adjacency matrix $\cW$, and given that $h(\cW)$ converges absolutely, it is decomposed as
	%
	\begin{equation}
		h(\cW) = U_1 g(\Lambda_1) U_1^\T + h(\cW - U_1 \Lambda_1 U_1^\T),
	\label{eq:2-main}
	\end{equation}
	%
	where
	%
	\begin{equation}
		g(A) \defn h(A) - h(\vO)
	\label{eq:2-aux}
	\end{equation}
	%
	for $n \times n$ real symmetric matrix $A$. For $h = h_\alpha$ and for $x \in [-1,1]$ in particular, $g_\alpha(x) \defn h_\alpha(x) - h_\alpha(0) = (1 - \alpha) \alpha x / (1 - \alpha x)$.
\end{theorem}

Observe that $\Lambda_2, U_2$ do not appear in~(\ref{eq:main}) and indeed it is only the largest $r$ eigenvalues $\Lambda_1$ and corresponding eigenvectors $U_1$ of $\cW$ that we need to compute.


==> ext-plots.tex <==
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{pgf,tikz}

\usepackage{tikzextern}
%\usepackage{pgffor}
\newcommand{\extfig}[2]{\tikzsetnextfilename{figs/extern/#1}{#2}}
\newcommand{\extdata}[1]{}


==> no-plots.tex <==
\newcommand{\extfig}[2]{!}
\newcommand{\extdata}[1]{}

